Special subvarieties arising from families of cyclic covers of the projective line

We consider families of cyclic covers of the projective line, where we fix the covering group and the local monodromies and we vary the branch points. We prove that there are precisely twenty such families that give rise to a special subvariety in the moduli space of abelian varieties. Our proof uses techniques in mixed characteristics due to Dwork and Ogus.

==> BMmacs <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% First part: fonts
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\catcode`\@=11
\def\hexnumber@#1{\ifcase#1 0\or1\or2\or3\or4\or5\or6\or7\or8\or9\or
        A\or B\or C\or D\or E\or F\fi }
%%
%%  Blackboard bold
%%
\font\tenmsa=msam10  \font\tenmsb=msbm10
\font\eightmsa=msam8 \font\eightmsb=msbm8
\font\sevenmsa=msam7 \font\sevenmsb=msbm7
\font\sixmsa=msam6   \font\sixmsb=msbm6
\font\fivemsa=msam5  \font\fivemsb=msbm5
\newfam\msafam
\textfont\msafam=\tenmsa  \scriptfont\msafam=\sevenmsa
  \scriptscriptfont\msafam=\fivemsa
\edef\msa@{\hexnumber@\msafam}
\newfam\msbfam
\textfont\msbfam=\tenmsb  \scriptfont\msbfam=\sevenmsb
  \scriptscriptfont\msbfam=\fivemsb
\edef\msb@{\hexnumber@\msbfam}
\def\Bbb{\ifmmode\let\next\Bbb@\else
        \def\next{\errmessage{Use \string\Bbb\space only in math 
mode}}\fi\next}
\def\Bbb@#1{{\Bbb@@{#1}}}
\def\Bbb@@#1{\fam\msbfam#1}
%%
%%  sans serif (sf)
%%
\font\tensf=cmss10
\font\eightsf=cmss8
\font\sevensf=cmss7
\font\sixsf=cmss6
\font\fivesf=cmss5
\newfam\sffam
\textfont\sffam=\tensf  \scriptfont\sffam=\sevensf
  \scriptscriptfont\sffam=\fivesf
\edef\sf@{\hexnumber@\sffam}
\def\sf{\let\next\sf@\next}
\def\sf@#1{\fam\sffam#1}
%%
%%  \bfit 
%%
\catcode`\@=11
\font\tenmib=cmmib10
\font\eightmib=cmmib8
\font\sevenmib=cmmib7
\font\sixmib=cmmib6
\font\fivemib=cmmib5
\newfam\mibfam
\textfont\mibfam=\tenmib  \scriptfont\mibfam=\sevenmib
  \scriptscriptfont\mibfam=\fivemib
\edef\mib@{\hexnumber@\mibfam}
\def\bfit{\ifmmode\let\next\bfit@\else
  \def\next{\errmessage{Use \string\bfit\space only in math mode}}\fi\next}
\def\bfit@#1{\fam\mibfam#1}
%%
%%  \frak (eufm)
%%
\font\teneufm=eufm10
\font\eighteufm=eufm8
\font\seveneufm=eufm7
\font\sixeufm=eufm6
\font\fiveeufm=eufm5
\newfam\eufmfam
\textfont\eufmfam=\teneufm  \scriptfont\eufmfam=\seveneufm
  \scriptscriptfont\eufmfam=\fiveeufm
\edef\eufm@{\hexnumber@\eufmfam}
\def\frak{\ifmmode\let\next\frak@\else
  \def\next{\errmessage{Use \string\frak\space only in math mode}}\fi\next}
\def\frak@#1{\fam\eufmfam#1}
%%
%%  RSFS
%%
\font\teneusm=rsfs10
\font\seveneusm=rsfs7
\font\fiveeusm=rsfs5
\newfam\eusmfam
\textfont\eusmfam=\teneusm  \scriptfont\eusmfam=\seveneusm
  \scriptscriptfont\eusmfam=\fiveeusm
\edef\eusm@{\hexnumber@\eusmfam}
\def\euscr{\ifmmode\let\next\euscr@\else
  \def\next{\errmessage{Use \string\euscr\space only in math mode}}\fi\next}
\def\euscr@#1{\fam\eusmfam#1}
%%
%% Special Math chars
%%
\mathchardef\square="0\msa@03
\mathchardef\myleq="3\msa@36
\mathchardef\mygeq="3\msa@3E
\let\leq=\myleq
\let\geq=\mygeq
\catcode`\@=12

%%
%% Fonts for 8-point
%%
\font\eightrm=cmr8  \font\sixrm=cmr6
\font\eighti=cmmi8  \font\sixi=cmmi6
\font\eightsy=cmsy8 \font\sixsy=cmsy6
\font\eightbf=cmbx8 \font\sixbf=cmbx6
\font\eighttt=cmtt8
\font\eightit=cmti8
\font\eightsl=cmsl8
\font\eighteusm=rsfs7 scaled\magstep1
\font\sixeusm=rsfs5 scaled\magstep1
%%
\catcode`@=11
\newskip\ttglue
\def\eightpoint{\def\rm{\fam0\eightrm}% switch to 8-point type
  \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\eighti  \scriptfont1=\sixi  \scriptscriptfont1=\fivei
  \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex   \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \textfont\itfam=\eightit  \def\it{\fam\itfam\eightit}%
  \textfont\slfam=\eightsl  \def\sl{\fam\slfam\eightsl}%
  \textfont\ttfam=\eighttt  \def\tt{\fam\ttfam\eighttt}%
  \textfont\bffam=\eightbf  \scriptfont\bffam=\sixbf
    \scriptscriptfont\bffam=\fivebf  \def\bf{\fam\bffam\eightbf}%
  \textfont\sffam=\eightsf  \scriptfont\sffam=\sixsf
    \scriptscriptfont\sffam=\fivesf  \def\sf{\fam\sffam\eightsf}%
  \textfont\msafam=\eightmsa \scriptfont\msafam=\sixmsa
    \scriptscriptfont\msafam=\fivemsa
  \textfont\msbfam=\eightmsb \scriptfont\msbfam=\sixmsb
    \scriptscriptfont\msbfam=\fivemsb \def\Bbb{\fam\msbfam\eightmsb}%
  \textfont\eufmfam=\eighteufm \scriptfont\eufmfam=\sixeufm
    \scriptscriptfont\eufmfam=\fiveeufm \def\frak{\fam\eufmfam\eighteufm}%
 \textfont\eusmfam=\eighteusm \scriptfont\eusmfam=\sixeusm
    \scriptscriptfont\eusmfam=\fiveeusm \def\euscr{\fam\eusmfam\eighteusm}%
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=10pt
  \setbox\strutbox=\hbox{\vrule height7pt depth2pt width0pt}%
  \let\sc=\sixrm \let\big=\eightbig \normalbaselines\rm}
\def\eightbig#1{{\hbox{$\textfont0=\ninerm\textfont2=\ninesy
  \left#1\vbox to6.5pt{}\right.\n@space$}}}
\catcode`@=12

%%
%% fonts for the title
%%
\font\namefont=cmr12
\font\byfont=cmti12
\font\titlefont=cmbx12
\font\sectitlefont=cmbx10


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Second part: layout, sections, counters
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%% PAGE SIZE and PAGE LAYOUT:
%%
\hsize16truecm
\vsize23.5truecm
\normalbaselineskip=13.5pt
\normalbaselines


%%
%% Various counters that are used for the chapters, sections etc
%%
\newcount\secno
\def\sectno{\number\secno}

\newcount\ssecno
\def\ssectno{\number\ssecno}

\newcount\referno
\def\refno{\number\referno}

\newcount\equano
\def\equatno{\number\equano}

\newcount\tablno\tablno=0
\def\tableno{\number\tablno}

\newcount\caseno\caseno=0
\def\casenr{{\number\caseno}}

%%
%% sections
%%
\def\section#1#2{%
\advance\secno by 1\ssecno=0\equano=0\definexref{#2}{\sectno}{section}%
\vskip2.0\bigskipamount plus 2pt minus 1pt%
\goodbreak\centerline{{\sectitlefont \sectno. #1}}%
\nobreak\ignorespaces}

\def\subsection{\advance\ssecno by 1\equano=0%
\vskip.75\bigskipamount plus 2pt minus 1pt%
\ifnum\ssecno>1\penalty-300\else\nobreak\fi%
\noindent{{\bf (\sectno.\ssectno)}}\enspace \ignorespaces}

\def\intro{%
\ssecno=0\equano=0%
\vskip2.0\bigskipamount plus 2pt minus 1pt%
\goodbreak\centerline{{\sectitlefont Introduction}}%
\nobreak\ignorespaces}

\def\introssect{\advance\ssecno by 1\equano=0%
\vskip.75\bigskipamount plus 2pt minus 1pt%
\ifnum\ssecno>1\penalty-300\else\nobreak\fi%
\noindent\ignorespaces}

\def\label#1{\definexref{#1}{\sectno.\ssectno}{subsection}}

%%
%% used for labels of references:
%%
\def\Reference#1{\advance\referno by1\definexref{#1}{\refno}{}\item{\rm [\refno]}}


%% The following macro is used for numbered equations. 
%%
\def\eqlabel#1{\global\advance\equano by 1%
\leqno{\hbox{\bf (\sectno.\ssectno.\equatno)}}%
\definexref{#1}{\sectno.\ssectno.\equatno}{}}




\newdimen\listindent
\listindent=20pt
\def\itemize{\begingroup 
\advance\leftskip by \listindent 
\parindent=-\listindent} 
\def\stopitemize{\par\endgroup} 
\def\item#1{\par\leavevmode 
\hbox to \listindent{#1\hfil}\ignorespaces 
} 

\let\iitem=\itemitem

\def\tablelabel#1{\global\advance\tablno by 1\definexref{#1}{\tableno}{}}

\def\Romno#1{\uppercase\expandafter{\romannumeral #1}}
\let\romno=\romannumeral

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Third part: maths
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%%  Blackboard Bold
%%
\def\mA{{\Bbb A}}
\def\mC{{\Bbb C}}
\def\mD{{\Bbb D}}
\def\mE{{\Bbb E}}
\def\mF{{\Bbb F}}
\def\mG{{\Bbb G}}
%\def\mH{{\Bbb H}}
\def\mL{{\Bbb L}}
\def\mM{{\Bbb M}}
\def\mN{{\Bbb N}}
\def\mP{{\Bbb P}}
\def\mQ{{\Bbb Q}}
\def\mR{{\Bbb R}}
\def\mS{{\Bbb S}}
\def\mV{{\Bbb V}}
\def\mZ{{\Bbb Z}}
%
\def\Af{\mA_\fin}
%%
%%  Script letters:
%%
%%
\def\cA{{\euscr A}}
\def\cD{{\euscr D}}
\def\cK{{\euscr K}}
\def\cM{{\euscr M}}
\def\cO{{\euscr O}}
\def\cQ{{\euscr Q}}
%%
%%  Fraktur:
%%
%%
\def\gH{{\frak H}}
\def\gp{{\frak p}}
\def\gS{{\frak S}}
%%
%%
%%  arrows
%%
%%
\def\stretcharrow{\mathop{\hbox to 15pt{\rightarrowfill}}}
\def\mapright#1{\mathrel{\stretcharrow\limits^{\;\,#1\;\;}}}
\def\jjoinrel{\mathrel{\mkern-3.3mu}}
\def\hooklongrightarrow{\lhook\jjoinrel\longrightarrow}
\let\longhookrightarrow=\hooklongrightarrow
\def\injmapright#1{\lhook\jjoinrel\mapright{#1}}
\def\isomarrow{\mapright{\sim}}
\def\twoheadrightarrow{\rightarrow\kern -8pt\rightarrow}

%%
%%
%%  "operator names"
%%
%%
\def\Aut{{\rm Aut}}
\def\Coker{{\rm Coker}}
\def\CSp{{\rm CSp}}
\def\End{{\rm End}}
%\def\Frob{{\rm Frob}}
\def\Frob{F}
\def\GL{{\rm GL}}
\def\Hdg{{\rm Hdg}}
\def\Jac{{\rm Jac}}
\def\Ker{{\rm Ker}}
\def\KS{{\rm KS}}
\def\Mono{{\rm Mon}}
\def\PGL{{\rm PGL}}
\def\PSp{{\rm PSp}}
\def\PSU{{\rm PSU}}
\def\PU{{\rm PU}}
\def\Res{{\rm Res}}
\def\SL{{\rm SL}}
\def\Spec{\mathop{\rm Spec}\nolimits}
\def\Sp{{\rm Sp}}
\def\SU{{\rm SU}}
\def\Sym{{\rm Sym}}
\def\UU{{\rm U}}

\def\ad{{\rm ad}}
\def\an{{\rm an}}
\def\can{{\rm can}}
\def\div{{\rm div}}
\def\even{{\rm even}}
\def\fin{{\rm fin}}
\def\gcd{{\rm gcd}}
\def\mult{{\rm mult}}
\def\new{{\rm new}}
\def\odd{{\rm odd}}
\def\old{{\rm old}}
\def\order{{\rm ord}}
\def\pr{{\rm pr}}
%%
 
\let\ol=\overline 

\let\tempcolon=\colon
\def\colon{\tempcolon\,}

\def\frpart#1{\left\langle #1\right\rangle}
\def\repr#1{[#1]}
\def\size#1{\left\vert#1\right\vert}

\def\Proof{\noindent{\it Proof.\/}\enspace}
\def\QED{\unskip\nobreak\hfill\hbox{\quad $\square$}}

%%
%% END OF MACRO FILE
%%
